BarrierBypass: Out-of-Sight Clean Voice Command Injection Attacks through Physical Barriers

The growing adoption of voice-enabled devices (e.g., smart speakers), particularly in smart home environments, has introduced many security vulnerabilities that pose significant threats to users' privacy and safety. When multiple devices are connected to a voice assistant, an attacker can cause serious damage if they can gain control of these devices. We ask where and how can an attacker issue clean voice commands stealthily across a physical barrier, and perform the first academic measurement study of this nature on the command injection attack. We present the BarrierBypass attack that can be launched against three different barrier-based scenarios termed across-door, across-window, and across-wall. We conduct a broad set of experiments to observe the command injection attack success rates for multiple speaker samples (TTS and live human recorded) at different command audio volumes (65, 75, 85 dB), and smart speaker locations (0.1-4.0m from barrier). Against Amazon Echo Dot 2, BarrierBypass is able to achieve 100% wake word and command injection success for the across-wall and across-window attacks, and for the across-door attack (up to 2 meters). At 4 meters for the across-door attack, BarrierBypass can achieve 90% and 80% injection accuracy for the wake word and command, respectively. Against Google Home mini BarrierBypass is able to achieve 100% wake word injection accuracy for all attack scenarios. For command injection BarrierBypass can achieve 100% accuracy for all the three barrier settings (up to 2 meters). For the across-door attack at 4 meters, BarrierBypass can achieve 80% command injection accuracy. Further, our demonstration using drones yielded high command injection success, up to 100%. Overall, our results demonstrate the potentially devastating nature of this vulnerability to control a user's device from outside of the device's physical space.

==> drone.tex <==
\section{\textcolor{red}{Drone-based Attack}}
\label{sec:drone}

\textcolor{red}{In this section, we demonstrate that the \aname attack can be launched \textit{remotely} via drone technology. Videos of the successful drone attack can be found on our website: \url{https://sites.google.com/view/barrierbypass}}

\subsection{\textcolor{red}{Equipment}}
\textcolor{red}{We utilized two drone models in our experiments. The first drone was a Toys-Sky S167 Quadcopter (``S167'')}~\cite{S167} \textcolor{red}{equipped with an SRS-XB2 Bluetooth speaker. The second drone was the Holy Stone HS700 (``HS700'')}~\cite{HS700} \textcolor{red}{equipped with an Anker Soundcore Bluetooth speaker. For all experiments we used a digital sound level meter to ensure the command audio played was at the correct volume. Additionally, we measured the loudness of each drone when it was turned on and prepared for flight (e.g., volume of the drones when the propellers were spinning). The S167 has an operating volume of 85 dB, and the HS700 has an operating loudness of 73 dB. Our experiments compromised simulated attacks targeting an Amazon Echo Dot 2 and Google Home smart speaker.}

\subsection{\textcolor{red}{Experimental Design}}
\textcolor{red}{Our first set of experiments utilized the S167 drone and demonstrated attacks targeting the Echo Dot smart speaker. Because of its louder volume during operation, we found that the command audio had to be increased from what was determined in prior experiments (without a drone). We recorded command injection success when the audio was played at 90 and 95 dB. The remaining experiments utilized the quieter HS700 drone and targeted both an Echo Dot and Google Home smart speaker. For all experiments, the drones were attached to the Bluetooth speakers, turned on and placed on the opposite side of the window from the smart speakers (Figure}~\ref{fig:drone_exp}).
	
\textcolor{red}{In these experiments we recorded command injection success when the audio was played at 85 dB (the same dB level used in earlier experiments without a drone). For all experiments we utilized the three TTS command samples that proved to have the highest performance from our earlier experiments in the Across-Window scenario (i.e., TTS-M1, TTS-M2 and TTS-F2). For each combination of audio sample and SPL, we attempted the command injection attack 10 times and recorded the number of successes.}

\subsection{\textcolor{red}{Results}}
Table~\ref{tab:drone_results} \textcolor{red}{depicts the results for each of the scenarios tested. Firstly, we found that using a drone with an operating loudness of 85 dB (S167) required command audio be played at 90+ dB. Specifically, at 90 dB we observed command injection success only up to 50\%. However, increasing the command audio to 95 dB allowed us to observe attack success up to 100\%. Since the operating loudness of the S167 was equal to the volume of audio used in our original experiments, the command audio in the presence of the drone had to be increase by at least 5 dB to overcome the added noise and achieve an SNR closer to 1.0 for successful command injection.}
	
\textcolor{red}{For our remaining experiments using the HS700 drone with a much lower operating loudness level, we observed high rates of command injection success, similar to what was observed in prior experiments when no drone was used. Because the operating loudness of the HS700 is only 73 dB, the 85 dB command audio level was not hindered by the added noise because it maintained a similarly high SNR. When targeting the Echo Dot, we observed attack success up to 100\%. And when targeting the Google Home we observed attack success up to 90\%.}

\begin{figure}[h]
	\captionsetup{font=footnotesize,labelfont=bf,width=0.9\linewidth}
	\centering
	\includegraphics[width=0.85\linewidth]{figs/drone_attack.pdf}
	\caption{\textcolor{red}{Image of drone attack simulated in our experimentation.}}
	\label{fig:drone_exp}
\end{figure}

%\begin{table*}[ht]
%	\captionsetup{font=footnotesize,labelfont=bf}
%	%\captionsetup{width=1\linewidth}
%	\centering
%	\caption{Command injection success rates observed during the drone experiments.}
%	%\vspace{-2mm}
%	\includegraphics[scale=0.62]{figs/drone_results.pdf}
%	%\vspace{-4mm}
%	\label{tab:drone_results}
%\end{table*}
